A Study of Gender Impact in Self-supervised Models for Speech-to-Text Systems

Self-supervised models for speech processing emerged recently as popular foundation blocks in speech processing pipelines. These models are pre-trained on unlabeled audio data and then used in speech processing downstream tasks such as automatic speech recognition (ASR) or speech translation (ST). Since these models are now used in research and industrial systems alike, it becomes necessary to understand the impact caused by some features such as gender distribution within pre-training data. Using French as our investigation language, we train and compare gender-specific wav2vec 2.0 models against models containing different degrees of gender balance in their pre-training data. The comparison is performed by applying these models to two speech-to-text downstream tasks: ASR and ST. Results show the type of downstream integration matters. We observe lower overall performance using gender-specific pre-training before fine-tuning an end-to-end ASR system. However, when self-supervised models are used as feature extractors, the overall ASR and ST results follow more complex patterns in which the balanced pre-trained model does not necessarily lead to the best results. Lastly, our crude 'fairness' metric, the relative performance difference measured between female and male test sets, does not display a strong variation from balanced to gender-specific pre-trained wav2vec 2.0 models.

==> tables/st_data_with_duration.tex <==
\begin{table}
\centering
\caption{Statistics for the \textit{fr-\{en,es,pt\}} mTEDx with gender annotation (M=male;F=female;B=speakers of both genders present in the talk).}
%Speech translation data. Number of talks and duration per gender for training, valid and test (training varies per lang. pair while valid and test are similar across lang. pairs). \textit{Both} means multiple (male and female) speakers within the talk.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{llcccc}\toprule
                                        &             & \textbf{M} & \textbf{F} & \textbf{B} & \textbf{ALL} \\\midrule
\multirow{2}{*}{\textbf{fr-en (train)}} & \# speakers & 146        & 102        & 2             & 250          \\
                                        & duration    & 26:28:11   & 18:14:12   & 0:22:24       & 45:04:45     \\
\multirow{2}{*}{\textbf{fr-es (train)}} & \# speakers & 110        & 86         & -             & 196          \\
                                        & duration    & 17:58:50   & 14:31:24   & -             & 32:30:13     \\
\multirow{2}{*}{\textbf{fr-pt (train)}} & \# speakers & 57         & 55         & -             & 112          \\
                                        & duration    & 10:39:16   & 9:22:44    & -             & 20:01:58     \\\midrule
\multirow{2}{*}{\textbf{All (valid)}}   & \# speakers & 5          & 7          & -             & 12           \\
                                        & duration    & 0:38:24    & 1:00:08    & -             & 1:38:32   \\\bottomrule
%discrepancy between segments and actual splited files
%\multirow{2}{*}{\textbf{All (valid)}}   & \# speakers & 5          & 7          & -             & 12           \\
%                                        & duration    & 0:43:39    & 1:04:52    & -             & 1:48:30     \\\bottomrule
\end{tabular}
}
\label{tab:stdata}
\end{table}
